Improved Algorithms for Misspecified Linear Markov Decision Processes

For the misspecified linear Markov decision process (MLMDP) model of Jin et al. [2020], we propose an algorithm with three desirable properties. (P1) Its regret after $K$ episodes scales as $K \max \{ \varepsilon_{\text{mis}}, \varepsilon_{\text{tol}} \}$, where $\varepsilon_{\text{mis}}$ is the degree of misspecification and $\varepsilon_{\text{tol}}$ is a user-specified error tolerance. (P2) Its space and per-episode time complexities remain bounded as $K \rightarrow \infty$. (P3) It does not require $\varepsilon_{\text{mis}}$ as input. To our knowledge, this is the first algorithm satisfying all three properties. For concrete choices of $\varepsilon_{\text{tol}}$, we also improve existing regret bounds (up to log factors) while achieving either (P2) or (P3) (existing algorithms satisfy neither). At a high level, our algorithm generalizes (to MLMDPs) and refines the Sup-Lin-UCB algorithm, which Takemura et al. [2021] recently showed satisfies (P3) for contextual bandits. We also provide an intuitive interpretation of their result, which informs the design of our algorithm.

==> linucbproof.tex <==
\section{Proposition \ref{propLinUcb} proof} \label{appLinUcbProof}

We essentially follow the existing proof . First, define the good event
\begin{equation}
\mathcal{G}' = \cap_{k=1}^K \left\{ \left\| \sum_{\tau=1}^{k-1} \phi(s^\tau,a^\tau) \eta^\tau \right\|_{ \Lambda_k^{-1} } \leq \sqrt{ 2 d \log ( (\lambda+K)/(\lambda \delta ) ) } \right\} .
\end{equation}
By Theorem 1 of \cite{abbasi2011improved}, the assumption on $\eta^\tau$, Lemma 10 of \cite{abbasi2011improved}, and the $\ell_2$ norm assumption on $\phi(s^\tau,a^\tau)$, $\P(\mathcal{G}') \geq 1-\delta$. We bound regret on $\mathcal{G}'$. Let $\Delta^\tau = r(s^\tau,a^\tau) - \phi(s^\tau,a^\tau)^\trans \theta$ denote the episode $\tau$ misspecification. Then if we define
\begin{align}
w_{k,1} = \Lambda_k^{-1} \sum_{\tau=1}^{k-1} \phi(s^\tau,a^\tau)  \phi(s^\tau,a^\tau)^\trans \theta  , \quad w_{k,2} = \Lambda_k^{-1} \sum_{\tau=1}^{k-1} \phi(s^\tau,a^\tau) \eta^\tau , \quad w_{k,3} = \Lambda_k^{-1} \sum_{\tau=1}^{k-1} \phi(s^\tau,a^\tau)  \Delta^\tau ,
\end{align}
we have $w_k = \sum_{i=1}^3 w_{k,i}$, which implies
\begin{equation}
| \phi(s,a)^\trans ( w_k - \theta ) | \leq | \phi(s,a)^\trans ( w_{k,1} - \theta ) | + | \phi(s,a)^\trans w_{k,2} | + | \phi(s,a)^\trans w_{k,3} | .
\end{equation}
Similar to the analysis of $z_2$ in the proof of Claim \ref{clmEstError}, we have
\begin{equation} \label{eqW1final}
| \phi(s,a)^\trans ( w_{k,1} - \theta ) | = \lambda | \phi(s,a)^\trans \Lambda_k^{-1} \theta | \leq \sqrt{\lambda} \| \phi(s,a) \|_{\Lambda_k^{-1}} .
\end{equation}
On the event $\mathcal{G}'$, we obtain
\begin{equation} \label{eqW2final}
| \phi(s,a)^\trans w_{k,2} | \leq \sqrt{ 2 d \log ( ( \lambda + K ) / ( \lambda \delta ) ) } \| \phi(s,a) \|_{\Lambda_k^{-1}} .
\end{equation}
Similar to analysis of $z_3$ in the proof of Claim \ref{clmEstError}, we know
\begin{align}
| \phi(s,a)^\trans w_{k,3} | \leq \epsmis \sqrt{K} \| \phi(s,a) \|_{\Lambda_k^{-1}}  .
\end{align}
Hence, combining the previous four inequalities, we have shown that on $\mathcal{G}'$,
\begin{equation}
| \phi(s,a)^\trans ( w_k - \theta ) | \leq \left( \sqrt{\lambda} + \sqrt{ 2 d \log ( ( \lambda + K ) / ( \lambda \delta ) ) }  + \epsmis \sqrt{K} \right) \| \phi(s,a) \|_{\Lambda_k^{-1}} \leq \alpha \| \phi(s,a) \|_{\Lambda_k^{-1}} ,
\end{equation}
where the second inequality is by choice of $\lambda$ and $\alpha$. Thus, by the misspecification assumption,
\begin{equation}
| r(s,a) - \phi(s,a)^\trans w_k | \leq | r(s,a) - \phi(s,a)^\trans \theta | + | \phi(s,a)^\trans ( \theta - w_k ) | \leq \epsmis + \alpha \| \phi(s,a) \|_{\Lambda_k^{-1}}  .
\end{equation}
Hence, by definition of the optimal policy and \texttt{Lin-UCB},
\begin{equation}
r(s^k,a_\star^k) \leq \max_{a \in \A} \left( \phi(s^k,a)^\trans w_k + \alpha \| \phi(s^k,a) \|_{\Lambda_k^{-1}} + \epsmis  \right)   \leq r(s^k,a^k) +  2 \alpha \| \phi(s^k,a^k) \|_{\Lambda_k^{-1}} + 2 \epsmis . 
\end{equation}
Substituting into the regret definition, then using Cauchy-Schwarz, \cite{abbasi2011improved}'s Lemma 11, and some simple eigenvalue bounds, we obtain
\begin{equation}
R(K) \leq 2 \alpha \sum_{k=1}^K \| \phi(s^k,a^k) \|_{\Lambda_k^{-1}} + 2 \epsmis K  \leq 2 \alpha \sqrt{ K d \log ( (\lambda+K)/K) } + 2 \epsmis K .
\end{equation}
Since $( \lambda + K ) / \lambda = 1 + K / ( 1 + \epsmis^2 K ) \leq 1 + \min \{ K , \epsmis^{-2} \}$, by definition of $\alpha$, we have
\begin{equation}
\alpha = O \left( \sqrt{ 2 d \log ( \min \{ K , \epsmis^{-2} \} / \delta ) } + \epsmis \sqrt{K} \right) .
\end{equation}
Combining and again using $( \lambda + K ) / \lambda \leq 1 + \min \{ K , \epsmis^{-2} \}$ yields the desired bound.




==> mainproofdetails.tex <==
\section{Theorem \ref{thmMain} proof details} \label{appMainProof}

\subsection{Regret bound details}

\begin{proof}[Proof of Claim \ref{clmTildeEpsrnd}]
The first bound follows from Holder's inequality, Algorithm \ref{algMain}, a standard norm equivalence, and Assumption \ref{assLin}:
\begin{equation}
| \phi(s,a)^\trans ( w_{h,l}^k - \tilde{w}_{h,l}^k ) | \leq \| \phi(s,a) \|_1 \| w_{h,l}^k - \tilde{w}_{h,l}^k \|_\infty \leq \sqrt{d} \| \phi(s,a) \|_2 \epsrnd \leq  \sqrt{d} \epsrnd .
\end{equation}
For the second bound, by similar logic, we have 
\begin{align}
| \phi(s,a)^\trans ( ( \Lambda_{h,l}^k )^{-1} - ( \tilde{\Lambda}_{h,l}^k )^{-1} ) \phi(s,a) | & \leq \sum_{i,j = 1}^d | \phi_i(s,a) | | \phi_j(s,a) | | ( ( \Lambda_{h,l}^k )^{-1} - ( \tilde{\Lambda}_{h,l}^k )^{-1} )_{ij} | \\
& \leq \| \phi(s,a) \|_1^2 \epsrnd \leq  d\| \phi(s,a) \|_2^2 \epsrnd \leq d \epsrnd ,
\end{align}
which implies that
\begin{align}
\| \phi(s,a) \|_{ (\Lambda_{h,l}^k )^{-1} } & \leq \sqrt{ | \phi(s,a)^\trans ( \tilde{\Lambda}_{h,l}^k )^{-1} \phi(s,a) | + | \phi(s,a)^\trans ( ( \Lambda_{h,l}^k )^{-1} - ( \tilde{\Lambda}_{h,l}^k )^{-1} ) \phi(s,a) | } \\
& \leq \| \phi(s,a) \|_{ (\tilde{\Lambda}_{h,l}^k )^{-1} } + \sqrt{ d \epsrnd } .
\end{align}
By symmetry, $\| \phi(s,a) \|_{ (\tilde{\Lambda}_{h,l}^k )^{-1} } \leq \| \phi(s,a) \|_{ (\Lambda_{h,l}^k )^{-1} } + \sqrt{d \epsrnd}$ as well, which completes the proof.
\end{proof}

\begin{clm} \label{clmEllPot}
For any $k \in [K]$, $h \in [H]$, and $l \in [L]$,
\begin{equation}
\sum_{\tau \in \Psi_{h,l}^k} \| \phi(s_h^\tau,a_h^\tau) \|_{ (\Lambda_{ h,l }^\tau )^{-1} }^2 \leq 2 \log ( \det  (\Lambda_{ h,l }^k ) / \det ( 16 I )  ) \leq 2 d \log ( 1 + | \Psi_{h,l}^k | / (16d) ) .
\end{equation}
\end{clm}
\begin{proof}
The first bound is a restatement of Lemma D.2 from \cite{jin2020provably}. The second follows from Lemma 10 of \cite{abbasi2011improved} and Assumption \ref{assLin}.
\end{proof}

\begin{proof}[Proof of Claim \ref{clmPsiBound}]
Since $\Psi_{h,l}^0 \subset \cdots \subset \Psi_{h,l}^K$, it suffices to prove the bound for $k = K$. By Algorithm \ref{algMain}, $\Psi_{h,l}^K$ is the set of episodes $k \in [K]$ for which $b_h^k(s_h^k) = 1$ and $l_h^k(s_h^k) = l$. By Algorithm \ref{algSub}, $b_h^k(s_h^k) = 1$ and $l_h^k(s_h^k) = l$ implies that $\| \phi(s_h^k,a_h^k) \|_{ (\tilde{\Lambda}_{ h,l }^k )^{-1} } > 2^{-l}$. Combined with Claim \ref{clmTildeEpsrnd}, and since $\epsrnd \leq 2^{-4l} / d \leq 2^{-2(l+1)} / d$ in Algorithm \ref{algMain}, we obtain
\begin{align}
1 & < 2^{2l} \| \phi(s_h^k,a_h^k) \|_{ (\tilde{\Lambda}_{ h,l }^k )^{-1} }^2 \leq 2^{2l+1} \| \phi(s_h^k,a_h^k) \|_{ ({\Lambda}_{ h,l }^k )^{-1} }^2 + 2^{2l+1} d \epsrnd  \leq 2^{2l+1} \| \phi(s_h^k,a_h^k) \|_{ ({\Lambda}_{ h,l }^k )^{-1} }^2 + 1/2 ,
\end{align}
or, after rearranging, $1 < 2^{2(l+1)} \| \phi(s_h^k,a_h^k) \|_{ ({\Lambda}_{ h,l }^k )^{-1} }^2$. Combined with Claim \ref{clmEllPot}, we obtain
\begin{equation} \label{eqPsiBoundInit}
|\Psi_{h,l}^K| = \sum_{k \in \Psi_{h,l}^K} 1 < 2^{2(l+1)} \sum_{k \in \Psi_{h,l}^K} \| \phi(s_h^k,a_h^k) \|_{ (\Lambda_{ h,l }^k )^{-1} }^2 \leq 2^{2l+3}  d \log ( 1 + |\Psi_{h,l}^K| / (16d) ) .
\end{equation}
Multiplying and dividing the right side of \eqref{eqPsiBoundInit} by $2$, we get
\begin{equation}
|\Psi_{h,l}^K| \leq 2^{2(l+2)} d \log \left( \sqrt{ 1 + |\Psi_{h,l}^K| / (16d) } \right) \leq 2^{2(l+2)} d \log \left( 1 + \sqrt{|\Psi_{h,l}^K| / (16d) } \right) \leq  2^{2 (l+1)} \sqrt{d |\Psi_{h,l}^K|} ,
\end{equation}
or, after rearranging,
\begin{equation} \label{eqPsiLooseBound}
|\Psi_{h,l}^K| \leq ( 2^{2(l+1)} \sqrt{d} )^2 = 2^{4(l+1)} d .
\end{equation}
Plugging \eqref{eqPsiLooseBound} into the right side of \eqref{eqPsiBoundInit}, we obtain
\begin{equation}
| \Psi_{h,l}^k | \leq 2^{2l+3} d \log ( 1 + 2^{4l} ) < 2^{2l+3} d \log ( 2 \cdot 2^{4l} ) \leq 2^{2l+3} d \log 2^{5l} < 2^{2l+3} d \cdot 5l = 40 \cdot 4^l d l . 
\end{equation}
Finally, since $40 < 64 = 2^6$ and $l \leq 2^{l-1}$ for any $l \in \N$, we have $40 \cdot 4^l  \cdot l < 2^6 \cdot 4^l \cdot 2^{l-1}  = 2^{3l+5}$.
\end{proof}

\begin{cor} \label{corDetRat}
For any $k \in [K]$, $h \in [H]$, and $l \in [L]$, $\det  (\Lambda_{ h,l }^k ) / \det ( 16 I ) \leq 2^{5dl}$.
\end{cor}
\begin{proof}
Combining Claims \ref{clmEllPot} and \ref{clmPsiBound}, we obtain
\begin{align}
 & \det  (\Lambda_{ h,l }^k ) / \det ( 16 I ) \leq ( 1 + | \Psi_{h,l}^k | / ( 16 d ) )^d \leq ( 1 + 2^{3 l + 1} )^d < ( 2 \cdot 2^{3l+1} )^d = 2^{ ( 3l+2) d } \leq 2^{5dl} . \qedhere
\end{align}
\end{proof}

\begin{cor} \label{corEllPot}
For any $k \in [K]$, $h \in [H]$, and $l \in [L]$, $\sum_{\tau \in \Psi_{h,l}^{k-1}} \| \phi(s_h^\tau,a_h^\tau) \|_{ (\Lambda_{ h,l }^k )^{-1} } \leq ( 2^l d )^4$.
\end{cor}
\begin{proof}
By Cauchy-Schwarz, Claim \ref{clmPsiBound}, and Lemma D.1 of \cite{jin2020provably},
\begin{align}
& \sum_{\tau \in \Psi_{h,l}^{k-1}} \| \phi(s_h^\tau,a_h^\tau) \|_{ (\Lambda_{ h,l }^k )^{-1} } \leq \sqrt{ | \Psi_{h,l}^{k-1} | \times \sum_{\tau \in \Psi_{h,l}^{k-1}} \| \phi(s_h^\tau,a_h^\tau) \|_{ (\Lambda_{ h,l }^k )^{-1} }^2 }  \leq \sqrt{ 2^{3l+5} d \times d } \leq 2^{ 4l } d \leq ( 2^l d )^4  . \qedhere
\end{align}
\end{proof}

\begin{clm} \label{clmNormEq}
For any $k \in [K]$, $h \in [H]$, $l \in [L]$, and $x \in \R^d$, $\| x \|_{ ( \Lambda_{h,l}^k )^{-1} } \leq \| x \|_2 / 4$.
\end{clm}
\begin{proof}
Let $\lambda_i \in [16,\infty)$ and $q_i \in \R^d$ denote the eigenvalues and eigenvectors of $\Lambda_{h,l}^k$. Then
\begin{align}
\| x \|_{ ( \Lambda_{h,l}^k )^{-1} }^2 & = \sum_{i=1}^d ( q_i^\trans x )^2 / \lambda_i \leq \sum_{i=1}^d ( q_i^\trans x )^2 / 16 = \| [q_1 \cdots q_d]^\trans x \|_2^2 / 16 = \| x \|_2^2 / 16 . 
\qedhere
\end{align}
\end{proof}

\begin{cor} \label{corExploratory}
For any $k \in [K]$, $h \in [H]$, and $s \in \S$ such that $b_h^k(s) = 1$, we have $l_h^k(s) > 1$.
\end{cor}
\begin{proof}
If instead $b_h^k(s) = l_h^k(s) = 1$, then by Algorithm \ref{algSub}, Claim \ref{clmTildeEpsrnd}, Claim \ref{clmNormEq}, Assumption \ref{assLin}, and definition $\epsrnd = 2^{-4L} / d$, we can find $a \in \A$ to obtain the following contradiction:
\begin{align}
& 1/2 < \| \phi(s,a) \|_{ ( \tilde{\Lambda}_{h,l}^k )^{-1} } \leq \| \phi(s,a) \|_{ ( \Lambda_{h,l}^k )^{-1} } + \sqrt{d \epsrnd} \leq ( \| \phi(s,a) \|_2 / 4 ) + 2^{-2L} \leq 1/2 . \qedhere
\end{align}
\end{proof}

\begin{clm} \label{clmWl2Bound}
For any $k \in [K]$, $h \in [H]$, and $l \in [L]$, $\| {w}_{h,l}^k \|_2 \leq ( 2^l d H )^4$.
\end{clm}
\begin{proof}
For any $x \in \R^d$, Claim \ref{clmNormEq} implies
\begin{equation}
\| ( \Lambda_{h,l}^k )^{-1} x \|_2 = \| ( \Lambda_{h,l}^k )^{-1/2} x \|_{ ( \Lambda_{h,l}^k )^{-1} } \leq \| ( \Lambda_{h,l}^k )^{-1/2} x \|_2 / 4 = \| x \|_{ ( \Lambda_{h,l}^k )^{-1} } / 4 .
\end{equation}
Combined with the triangle inequality and Corollary \ref{corEllPot}, we obtain
\begin{align}
\| w_{h,l}^k \|_2 & \leq \frac{1}{4} \sum_{ \tau \in \Psi_{h,l}^{k-1} } \| \phi(s_h^\tau,a_h^\tau) \|_{ ( \Lambda_{h,l}^k )^{-1} } | r_h^\tau(s_h^\tau,a_h^\tau) + V_{h+1}^k ( s_{h+1}^\tau )  | \\
& < H \sum_{ \tau \in \Psi_{h,l}^{k-1} } \| \phi(s_h^\tau,a_h^\tau) \|_{ ( \Lambda_{h,l}^k )^{-1} }  \leq H ( 2^l d )^4 \leq ( 2^l d H )^4 ,
 \end{align}
where the second inequality holds because $r_h^\tau(s_h^\tau,a_h^\tau) \in [0,1]$ by assumption and $V_{h+1}^k ( s_{h+1}^\tau ) \in [0,H]$ by definition in Algorithm \ref{algSub} (so $| r_h^\tau(s_h^\tau,a_h^\tau) + V_{h+1}^k ( s_{h+1}^\tau )  | \leq 1+H\leq 2H < 4H$).
\end{proof}

\begin{clm} \label{clmBetaBound}
Define $\mathcal{V}$ as in the proof of Lemma \ref{lemConcentration}. Then for any $k \in [K]$, $h \in [H]$, and $l \in [L]$,
\begin{equation}
\sqrt{ 8 H^2 \log \left(  \frac{ \det ( \Lambda_{h,l}^k ) }{ \det ( 16 I )} \frac{2 H L |\mathcal{V}|}{\delta} \right) } \leq \beta .
\end{equation}
\end{clm}
\begin{proof}
We first bound $|\mathcal{V}|$. Clearly, $|\mathcal{V}| \leq |\mathcal{X}|^L |\mathcal{Y}|^L$. Next, observe
\begin{equation}
|\mathcal{Y}| = ( 1 + 2 \ceil{ 1 / ( 16 \epsrnd ) } )^{d^2} \leq ( 3 + 1 / ( 8 \epsrnd ) )^{d^2} < 1/  \epsrnd^{d^2} = 2^{4 L d^2} d^{d^2} ,
\end{equation}
where the second inequality holds since $\epsrnd < 7/24$ in Algorithm \ref{algMain}. For $\mathcal{X}$, we have
\begin{align}
|\mathcal{X}| & \leq ( 3 + 2 ( 2^L d H )^4 / \epsrnd )^d \leq ( ( 3 \cdot 2^{-4} + 2 ) ( 2^L d H )^4 / \epsrnd )^d \\
& < ( 4 ( 2^L d H )^4 / \epsrnd )^d = 2^{( 8 L + 2) d } d^{5d} H^{4d} ,
\end{align}
where the second inequality uses $\epsrnd \leq 1$ in Algorithm \ref{algMain}. Hence, we have shown
\begin{equation}
| \mathcal{V} | \leq  ( 2^{4 L d^2} d^{d^2} \cdot 2^{ (8L+2) d } d^{5d} H^{4d} )^L \leq ( 2^{14} d^6 H^4 )^{L^2 d^2} .
\end{equation}
Furthermore, by Corollary \ref{corDetRat}, we have $\det ( \Lambda_{h,l}^k ) / \det ( 16 I ) \leq  2^{5dl} \leq 2^{ 5 L^2 d^2 }$. Combining,
\begin{equation}
\log \left( \frac{2 H L}{\delta} \cdot \frac{ \det ( \Lambda_{h,l}^k ) |\mathcal{V}| }{ \det ( 16 I )} \right) \leq \log \left( \frac{ 2 H L  }{\delta } \cdot ( 2^{19} d^6 H^4 )^{L^2 d^2}  \right) \leq 20 L^2 d^2 \log ( 2 d H L / \delta ) .
\end{equation}
Combining with the fact that $8 \cdot 20 = 160 < 169 = 13^2$, we obtain
\begin{align}
& \sqrt{ 8 H^2 \log \left(  \frac{ \det ( \Lambda_{h,l}^k ) }{ \det ( 16 I )} \frac{2 H L |\mathcal{V}|}{\delta} \right) } < 13 d H L \sqrt{ \log(3dHL/\delta) } = \beta . \qedhere
\end{align}
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemEstErrorLearner}]
We fix $k$ and use induction on $h$. When $h = H$, since $V_{H+1}^k(\cdot) = 0$, we have $\gamma_H^k = 0$ and $V_H^{\pi_k}(s) = r_H ( s , \pi_H^k(s) ) = \bar{Q}_H^k(s , \pi_H^k(s) )$ (for any $s$). Therefore, by Claim \ref{clmEstErrorLearner}, for any $s$,
\begin{align}
V_H^k (s) - V_H^{\pi_k}(s) = V_H^k(s) - \bar{Q}_H^k(s , \pi_H^k(s) ) \leq 8 \alpha \cdot 2^{-l_H^k(s)} b_H^k(s) + 2^{2-L} \alpha + \epseff . 
\end{align}
Hence, choosing $s = s_H^k$ yields the desired bound. Now assume \eqref{eqRecursion} holds for some $h+1 \in \{2,\ldots,H\}$. Then for any $s \in \S$,
\begin{align}
V_h^k(s) - V_h^{ \pi_k }(s)&= V_h^k(s) - \bar{Q}_h^k(s, \pi_h^k(s) ) + \int_{ s' \in \S } ( V_{h+1}^k(s') - V_{h+1}^{\pi_k}(s')  ) P_h( s' | s , \pi_h^k(s) ) \\
& \leq 8 \alpha \cdot 2^{-l_h^k(s)} b_h^k(s) + 2^{2-L} \alpha + \epseff + \int_{ s' \in \S } ( V_{h+1}^k(s') - V_{h+1}^{\pi_k}(s')  ) P_h( s' | s , \pi_h^k(s) ) ,
\end{align}
where the inequality again uses Claim \ref{clmEstErrorLearner}. Choosing $s = s_h^k$ and using the fact that $a_h^k = \pi_h^k(s_h^k)$ and the inductive hypothesis, we thus obtain
\begin{align}
V_h^k(s_h^k) - V_h^{ \pi_k }(s_h^k) & \leq 8 \alpha \cdot 2^{-l_h^k(s_h^k)} b_h^k(s_h^k) + 2^{2-L} \alpha + \epseff + \gamma_h^k+ V_{h+1}^k(s_{h+1}^k) - V_{h+1}^{ \pi_k }(s_{h+1}^k) \\
& \leq 8 \alpha \sum_{h'=h}^H 2^{ - l_{h'}^k(s_{h'}^k) } b_{h'}^k(s_{h'}^k) + \sum_{h'=h}^H \gamma_{h'}^k + ( 2^{2-L} + \epseff ) ( H - h + 1 ). \qedhere
\end{align}
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemOptimism}]
We again use induction on $h$. For $h = H$, the bound follows immediately from Claim \ref{clmOptimismH} and $V_{H+1}^\star(\cdot) = V_{H+1}^k(\cdot) = 0$. Now assume that for some $h+1 \in \{2,\ldots,H\}$ and all $s' \in \S$,
\begin{equation}
V_{h+1}^\star(s') - V_{h+1}^k(s')  \leq 2 L \epseff ( H - h )  .
\end{equation}
Combining this bound with Claim \ref{clmOptimismH}, for any $s \in \S$, we obtain
\begin{align}
V_h^\star(s) - V_h^k(s) & \leq \max \left\{ \max_{ a \in \A } \int_{s' \in \S} ( V_{h+1}^\star(s') - V_{h+1}^k(s') ) P_h(s'|s,a)  + 2 L \epseff , 0 \right\} \\
& \leq \max \left\{ 2 L \epseff (H-h) + 2 L \epseff , 0 \right\} = 2 L \epseff  ( H - h + 1 ) . \qedhere
\end{align}
\end{proof}

\subsection{Complexity analysis}

The time complexity of Algorithm \ref{algSub} is dominated by the computation of the set of induced norms $\{ \| \phi(s,a) \|_{ ( \tilde{\Lambda}_{h,l}^k )^{-1} } : a \in \A_{h,l}^k(s) , l \in [ l_h^k(s) ] \}$, which is at most $O(d^2 L |\A|)$. At episode $k$ of Algorithm \ref{algMain}, Algorithm \ref{algSub} is called to compute $\{ V_{h+1}^k(s_{h+1}^\tau) : \tau \in \Psi_{h,l}^{k-1} , l \in [L] , h \in \{2,\ldots,H\} \}$ in Line \ref{lnWeightVector} and $\{ \pi_h^k(s_h^k) : h \in [H] \}$ in Line \ref{lnTakeAction}, for a total number of calls
\begin{equation}
\sum_{h=2}^H \sum_{l=1}^L | \Psi_{h,l}^{k-1} | + H \leq 40 d H L \sum_{l=1}^L 4^l + H = O ( 4^L d H L ) ,
\end{equation}
where the inequality uses Claim \ref{clmPsiBound}. Alternatively, since $\cup_{l=1}^L \Psi_{h,l}^{k-1} \subset [K]$ for each $h \in [H]$, we can simply bound the number of calls by $O( HK )$. Hence, during each episode, the time complexity of all Algorithm \ref{algSub} calls is bounded above by
\begin{equation} \label{eqTimeCompInit}
O( d^2 H L |\A| \min\{ 4^L d L , K \} )  .
\end{equation}
Besides these calls, by a similar argument, computing the summations in Line \ref{lnWeightVector} has runtime at most $d \min \{ \sum_{h=1}^H \sum_{l=1}^L | \Psi_{h,l}^{k-1} | , HK \}  = O ( d H  \min \{ 4^L d L  , K \} )$, which is dominated by \eqref{eqTimeCompInit}. Iterative updates of $\Lambda_{h,l}^k$ and $(\Lambda_{h,l}^k)^{-1}$ and the rounding in Line \ref{lnRound} both have complexity $O(d^2 HL)$ per episode, and maintaining the sets $\Psi_{h,l}^k$ has complexity $O(H)$; both quantities are dominated by \eqref{eqTimeCompInit}. Hence, Algorithm \ref{algMain}'s per-episode runtime is
\begin{equation}
O ( d^2 H L |\A| \min\{ 4^L d L , K \} ) = O  \left( d^2 H |\A|  \min \left\{ d^2 \log( \tfrac{d}{\epstol} ) / \epstol^2 , K \right\} \log ( \tfrac{d}{\epstol} ) \right) .
\end{equation}

At episode $k$, Algorithm \ref{algMain} uses $\{ \Lambda_{h,l}^k \}_{ h \in [H] , l \in [L] }$ and $\{ w_{h,l}^k \}_{ h \in [H] , l \in [L] }$, and their rounded versions, which requires $O(d^2 H L)$ storage. Note these can be overwritten across episodes, so the total storage is $O(d^2 H L)$ as well. Additionally, at episode $k$, it needs to store $r_h^\tau(s_h^\tau,a_h^\tau)$ and $\{ \phi(s_h^\tau,a) \}_{a \in \A}$, for each $\tau \in \Psi_{h,l}^{k-1}$, $h \in [H]$, and $l \in [L]$. Similar to above, this storage can be bounded by either $d|\A| HK$ or $d|\A| \sum_{h=1}^H \sum_{l=1}^L | \Psi_{h,l}^{k-1} | = O ( 4^L d^2 H L |\A|  )$. Hence, the total space complexity is
 \begin{equation}
O ( d^2 H L + d H |\A| \min \{ 4^L d L  , K \} ) = O \left( d^2 H \log(\tfrac{d}{\epstol}) + d H |\A| \min \left\{ d^2 \log ( \tfrac{d}{\epstol} ) / \epstol^2 , K \right\} \right) .
\end{equation}


